GEVRM: Goal-Expressive Video Generation Model For Robust Visual Manipulation

With the rapid development of embodied artificial intelligence, significant progress has been made in vision-language-action (VLA) models for general robot decision-making. However, the majority of existing VLAs fail to account for the inevitable external perturbations encountered during deployment. These perturbations introduce unforeseen state information to the VLA, resulting in inaccurate actions and consequently, a significant decline in generalization performance. The classic internal model control (IMC) principle demonstrates that a closed-loop system with an internal model that includes external input signals can accurately track the reference input and effectively offset the disturbance. We propose a novel closed-loop VLA method GEVRM that integrates the IMC principle to enhance the robustness of robot visual manipulation. The text-guided video generation model in GEVRM can generate highly expressive future visual planning goals. Simultaneously, we evaluate perturbations by simulating responses, which are called internal embeddings and optimized through prototype contrastive learning. This allows the model to implicitly infer and distinguish perturbations from the external environment. The proposed GEVRM achieves state-of-the-art performance on both standard and perturbed CALVIN benchmarks and shows significant improvements in realistic robot tasks.

==> ICLR_2025_Template/includes/_introduction.tex <==
\section{Introduction}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% dpx: # dpx: v3

% With the recent surge in robotics and embodied AI, significant progress has been made in general visuomotor control. 
% However, most existing control policies are trained in idealized environments, without accounting for the inevitable external disturbances encountered during deployment. 
% Consequently, these policies struggle to accurately and reliably estimate the robot’s state, hindering the generation of robust and stable actions, and resulting in a significant decline in performance.
% Inspired by the principles of classical internal model control, we propose the Robot Intrinsic Model visuomotor Control (RoboIMC) method. 
% It integrates internal models to achieve precise estimation of the robot’s state, thereby enhancing the robustness of its actions. 
% RoboIMC comprises a text-conditioned video diffusion model for generating accurate visual plan states as reference inputs, two visual internal encoders for simulating responses, and a feedback-driven controller for action generation.
% Our method achieves state-of-the-art results on both standard and environmentally disturbed CALVIN benchmarks, and also shows significant improvements in realistic robotics tasks.

% 1: 引入general visuomotor control，列举一些例子
Robotics and embodied generalists have gained remarkable progress in recent years, with the successful advancement of large-scale data collection~\citep{vuong2023open}, universal state representation learning~\citep{li2023vision,du2024learning} and expressive policy learning~\citep{brohan2022rt,chi2023diffusion}, \textit{etc}. 
%
The above policies have proven effective in estimating the robot’s state and generating robust action in diverse environments, from physical simulators~\citep{mu2021maniskill,ding2023quar} to real-world settings meticulously designed.
% 
However, these meticulously designed environments don't account for the inevitable external disturbances encountered during deployment, e.g., fluctuated lighting conditions or noise video streams due to signal transmission issues.
%
When deployed in these non-ideal environments, the above visuomotor policy may struggle to accurately and reliably estimate the robot’s state, hindering the generation of robust and stable actions and resulting in a significant decline in performance.
% 
Consequently, deploying robots in scenarios with inevitable external disturbances remains a persistent challenge~\citep{}.


%
Some literature
have attempted to tackle the problem with large language models, splitting a prolonged job into detailed instructions for each minor movement~\citep{}, or sub-goals.
%
Though effective in high-level descriptions, texts could still be inadequate for detailed descriptions of the environment and robot state, leading to considerable issues under cross-morphology or multi-environments~\citep{du2024learning}.
Therefore, 
recent efforts have started embracing vision as a universal medium
to develop an embodied agent capable of planning diverse tasks through imagination and execution~\citep{black2023zero, du2024learning, Yang2023LearningIR}. These approaches involve a generative model for predicting future videos or goal images, followed by a goal-conditioned policy for translating the visual plan into actual actions. 
%
% Despite their successes, these methods often rely on idealized evaluation paradigms, where robot actions are executed in controlled environments without disturbances.
% %
% In real-world scenarios, however, lighting conditions may fluctuate, and video streams may suffer from noise due to signal transmission issues. 
% %
% Such subtle variations in non-ideal environments can lead to incorrect subgoal planning by the visual planner and imprecise execution by the goal-conditioned policy. Consequently, these challenges impose higher demands on the generalization capabilities of both the visual planner and the goal-conditioned policy.





% However, despite the promising results demonstrated by these approaches in controlled evaluation benchmarks, we have identified a critical limitation: these evaluations often assume an idealized perception environment that remains static throughout the testing process. Unfortunately, this assumption does not hold in real-world scenarios, where conditions such as dynamic lighting changes or subtle variations in camera positioning can cause substantial performance degradation.




% 2: 讲一些现有的局限性
% However, most existing control policies are trained in idealized environments, without accounting for the inevitable external disturbances encountered during deployment. 

% 3: 问题是struggle to accurately and reliably estimate the robot’s state，hindering the generation of robust and stable actions，resulting in a significant decline in performance

% 3: 讲解classical internal model control

% 4: 提出我们的方案


% 











%
% Some literature
% have attempted to tackle the problem with large language models, splitting a prolonged job into detailed instructions for each minor movement~\citep{}, or sub-goals.
% %
% Though effective in high-level descriptions, texts could still be inadequate for detailed descriptions of the environment and robot state, leading to considerable issues under cross-morphology or multi-environments~\citep{du2024learning}.
% Therefore, 
% recent efforts have started embracing vision as a universal medium
% to develop an embodied agent capable of planning diverse tasks through imagination and execution~\citep{black2023zero, du2024learning, Yang2023LearningIR}. These approaches involve a generative model for predicting future videos or goal images, followed by a goal-conditioned policy for translating the visual plan into actual actions. 
% %
% Despite their successes, these methods often rely on idealized evaluation paradigms, where robot actions are executed in controlled environments without disturbances.
% %
% In real-world scenarios, however, lighting conditions may fluctuate, and video streams may suffer from noise due to signal transmission issues. 
% %
% Such subtle variations in non-ideal environments can lead to incorrect subgoal planning by the visual planner and imprecise execution by the goal-conditioned policy. Consequently, these challenges impose higher demands on the generalization capabilities of both the visual planner and the goal-conditioned policy.

%








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% dpx: v1--素材

% general robotic simulator
% RoboSora: a learned simulator for general purpose robotics
% a robotics world model that understands contact physics and generates high fidelity video- towards a robot that plans, evaluated, and simulates in its own neural space.

% first proof of robot data significantly advancing scaling laws.

% 这个世界模型还能预测非平凡物体（如刚体）的相互作用、掉落物体的影响、部分可观测性、可变形物体（窗帘、衣物）和铰接物体（门、抽屉、窗帘、椅子）。

% 泛化性的能力是重要的
% 现有的方案，主要分为两套方案：显式和隐式的
% 隐式的方法受限于机器人的数据集的问题（高质量数据对缺失），显式的方法虽然解决了这类的问题，但是还有两个问题：
% 感知模型的通用性很成问题

% 下层模型的逆运动学的动作映射也很成问题

% 

% 扩充成一段：
% 世界模型解决了构建通用机器人时一个非常实际、但经常被忽视的挑战，即评估。如果你训练的机器人可以执行 1000 项任务，与先前模型相比，我们也很难确定新模型用在机器人上，在这 1000 项任务上表现优越。由于周围环境如光照细微的变化，即使模型权重相同，机器人也可能在几天内经历性能的快速下降。
% 如果环境随着时间的推移不断变化，那么此前在该环境中达到的实验性能很难复现，因为旧环境不存在了。如果你在不断变化的环境（如家庭或办公室）中评估多任务系统，那么这个问题将会变得更加糟糕。这一状况使得在现实世界中进行机器人科学研究变得异常困难。

% 借鉴一下1X的写法，现在的模型虽然可以用，但是在
% 实际应用过程中，由于场景的泛化性问题啊，性能往往会有很大的drop



% 机器人对于

% 机器人对广泛任务的通用性很关注
% For robots to be practical and useful, they must be general
% to the wide variety of conditions they will encounter in the
% world. 
% 因此激烈了机器人社区对于泛化性的追求
% It therefore has been of great interest in the robotics community to apply various recipes, such as larger datasets, more general model architecture, better explainable， to achieve broad generalization.
% 但是，尽管这些工作在评估的指标上很promising, 但是我们发现一个很重要的问题：这些评估过程往往假设是理想的感知环境，这种环境在各种评估过程中往往保持完全不变。不幸的是，这个假设在实际应用过程中往往是不成立的。比如说，开放环境下的光照的实时变化，相机位置设定的细微角度变化，都会给最终的性能带来巨大的drop.
%
% 如图表XXX所示，我们测试了现有一些SOTA方法对于这些变化的性能drop情况。我们可以发现，大部分的implict的工作，由于图像信息被压缩，天然损失了对于图像更好的理解能力，即使有工作提出希望借由预训练的video模型提升模型的性能, 但是我们发现这类工作因为训练的数据集有限，没有internet级别的数据集的训练，模型无法处理这些物理规律的变化。究其原因，这类模型缺少了对于感知世界的通用理解能力，这进一步限制了模型面向更通用的应用场景下。


% 为此，我们在这篇工作，想要探索 a general robotics world model that understands contact physics and generates high fidelity video- towards a robot that plans, evaluated, and simulates in its own neural space.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% dpx: v2



% For robots to be practical and useful, they must be general to the wide variety of conditions they will encounter in the world. 

% There has been significant interest in the robotics community to improve generalization by employing various strategies, such as leveraging larger models~\citep{alayrac2022flamingo}.

% % 得益于数据集的captures much of the complexity and variation in the domain that models will need to reason about

% % 但是这些工作都需要非常大量的pair的数据去训练，后面大家开始转向通用的world model 学习，因为这种方式可以跨越不同的数据集，不同的action space, 因而可以很好地泛化。

% % 其中，最经典的范式就是通过语言条件和当前的image去生成未来的一连串视频。

% % 这类工作在一些简单的arrangement上表现得很好，但是在涉及到长时序的任务上时候表现得一般

% % 究其原因是其时序视频的生成质量太差，导致整体性能变化得很大

% % 后面有哥们通过了只预测未来的帧来解决这个问题，在长时序的任务上表现得很好

% % 但是这种范式会导致很严重的泛化问题。

% % 在真实的环境受到干扰的情况下，SuSIE的鲁棒性会差很多

% % 由于缺乏了这种渐进式的推理过程，执行的鲁棒性下降了很多

% % 因此，本文想要探索一个更好地生成视频，且执行鲁棒性更强的世界模型理解器。


% % 

% % 在Sora和LLM都产生了大量的工作赋能了泛化性的提升

% % 尽管有大量的基于LLM的模型出现了，也提高了模型的整体感知能力，但是这类工作仍然受限于一个问题啊，就是说模型是从语言端解决问题的，需要大量的robot data去训练

% % 需要将感知空间对齐到机器人的action 空间

% % 这是需要大量的数据pair的

% % 由于不同的环境的action space什么的都不一样，因此

% % 但是这种方式

% % 先前的工作


% Consequently, there has been significant interest in the robotics community to improve generalization by employing various strategies, such as scaling up datasets~\citep{brohan2022rt}, designing more general model architectures~\citep{alayrac2022flamingo}, and enhancing explainability~\citep{du2024learning}.

% However, despite the promising results demonstrated by these approaches in controlled evaluation benchmarks, we have identified a critical limitation: these evaluations often assume an idealized perception environment that remains static throughout the testing process. Unfortunately, this assumption does not hold in real-world scenarios, where conditions such as dynamic lighting changes or subtle variations in camera positioning can cause substantial performance degradation.
% %
% As shown in \textcolor{red}{Figure 1}, we evaluated the performance drop of SOTA methods under these varying conditions. Our findings reveal that many \textcolor{red}{implicit models}, which rely on compressed image information, inherently lose the ability to fully understand the visual context. Although some approaches attempt to improve performance by using pre-trained video models, these models are constrained by the limited size of their training datasets, which are not on the scale of internet-level data. As a result, they struggle to handle changes governed by fundamental physical laws. {The core issue is that these models lack a general understanding of the perceptual world, which restricts their applicability to more generalized real-world scenarios.}

% To address these limitations, in this work, we propose \textcolor{red}{a robotics world model} that understands contact physics and generates high fidelity video towards a robot that plans, evaluated, and simulates in its own neural space.
% Specifically, 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% zhy: v1
% In the fields of computer vision and natural language processing (NLP), the current dominant paradigm is to build general models that can solve a wide variety of tasks. 
% Excellent zero-shot learning capabilities have emerged in some large pre-trained models \citep{chowdhery2023palm,hoffmann2022training,radford2021learning,alayrac2022flamingo}. 
% Inspired by the success of these studies, the field of robot learning is also building a large number of datasets of various decision-making tasks in different environments and striving to build general robot agents.

% Building a general model that can solve a variety of robot tasks is an important research issue in the field of robot learning. 
% The primary challenge is that the collection of paired vision, language, and robot expert actions is time-consuming and laborious. 
% Although there are some public robot decision-making task datasets \citep{mees2022calvin,walke2023bridgedata,vuong2023open,khazatsky2024droid}, the amount of data is still far from the massive text data on the Internet used in the field of NLP. 
% Some previous studies \citep{brohan2022rt,reed2022generalist} collected paired vision, language, and action data and trained an agent for solving long-term tasks. 
% Some other studies \citep{li2022pre,driess2023palm,kim2024openvla}  utilized the specific robot demonstrations to fine-tune large language models (LLMs) for visual and language inputs.
% However, due to the limited data size, these agents can only generalize within a limited data distribution and are difficult to expand to new environments and tasks that have never been seen before.

% Moreover, the diversity of environments and tasks in robot decision-making tasks also poses a severe challenge to training general robot agents. 
% Different decision-making tasks have different state-action spaces and environmental dynamic models. 
% Perceptual representation, knowledge sharing, and skill generalization across tasks and environments are greatly hindered. 
% % To alleviate this problem, the work \citep{reed2022generalist} argued that different environments and tasks can be encoded by utilizing universal tokens in a sequence modeling framework. 
% % However, it is unclear whether this approach can retain the rich semantic knowledge in the pre-trained model and efficiently transfer this knowledge to downstream robot tasks.
% To alleviate this problem, some works \citep{ajay2024compositional,du2024learning,black2023zero} fine-tune the language-conditioned video (or image) prediction model on robot data to obtain a robot behavior planner, and then utilize the goal-conditioned policy (or inverse dynamics model) to predict the robot's action. 
% However, the current model still has room for improvement in robot trajectory videos (and images). 
% These methods have difficulty simulating the physical characteristics of complex scenes in long-term tasks, and may even produce hallucinations of objects or actions that are unreal or do not exist in the physical world. 
% Therefore, inspired by the recent success of advanced text-conditioned video models \citep{videoworldsimulators2024,esser2024scaling} in greatly improving the quality of image and video generation, we leverage the diffusion transformer structure with more powerful expression capabilities and the efficient generation method rectified flow \citep{liu2022flow} to model and train the robot behavior planner.

% On the other hand, previous methods have the problem of inconsistency between behavior video (or image) inference and action prediction during the test phase. 
% This is because the  goal-conditioned policy utilizes future images in real data as goals during training, while only future images inferred by the behavior planner can be obtained during testing. 
% The difference between real images and generated images will lead to inaccurate action prediction. 
% To alleviate this discrepancy, we utilize contrastive learning to enhance the robustness of the image representation of the goal-conditioned policy so that it generalizes better to new environments. 
% Specifically, if the observation image and the goal image in a batch come from the same trajectory, they are positive samples, otherwise they are negative samples. 
% These pairs are optimized by swapping assignment tasks similar to \citep{caron2020unsupervised}.

% % In this work, we propose a new robot behavior planning model conditioned on abstract language text instructions and historical video trajectories. 
% % It utilizes text instructions as a universal interface for expressing task descriptions and utilizes the robot's sequential decision videos as a universal interface for conveying observed behaviors and actions in different environments and tasks. 
% % It generates the robot's future trajectory in the form of an image sequence conditioned on the robot's historical trajectory video and text instructions describing the current goal. 
% % Meanwhile, we also construct an inverse dynamics model as the goal-conditioned policy to predict actions. 
% % It utilizes the robot's historical decision videos and future images generated by the behavior planning model as a universal interface for conveying observed behaviors and goals in different environments and tasks.

% % Therefore, the robot behavior planning model and inverse dynamics model we constructed together form a hierarchical policy framework, which is characterized by the decoupling of environmental perception and decision-making actions under long-term decision-making tasks of robots. 
% % This decoupling helps to enhance the robot's general and robust decision-making control capabilities. 
% % The reason is that the upper-level behavior planning model can retain the massive knowledge of the video generation model pre-trained on a large-scale text video dataset, which can deepen the robot's perception of environmental objects and its understanding of the physical laws of the world. 
% % The model not only understands the specific content required by the abstract text instructions, but also understands the existence and operation of these things in the physical world. 
% % Moreover, the rich combinatorial nature of language instructions can also be utilized to synthesize new combined behaviors in many different environments and tasks. 
% % For specific downstream robot decision-making tasks, the training of the lower-level inverse dynamics model only requires a small number of robot action trajectories without text annotations.

% The main contribution of our work is to establish a new robot behavior planning model, which realizes accurate inference and reasonable planning of robot behavior for long-horizon tasks, and enhances the robot's deep perception and understanding of the underlying operation mode of the physical world.
% Moreover, the proposed representation enhancement method enables the goal-reaching policy to predict more accurate actions and achieve general and robust robot decision-making.
% Extensive experiments show that our method outperforms baseline methods in terms of robot behavior trajectory video generation quality and decision task success rate.
% Therefore, further extending our robot behavior planning model is a promising way to build a general robot agent in the physical world.

